IPC-Net: 3D point-cloud segmentation using deep inter-point convolutional layers

Over the last decade, the demand for better segmentation and classification algorithms in 3D spaces has significantly grown due to the popularity of new 3D sensor technologies and advancements in the field of robotics. Point-clouds are one of the most popular representations to store a digital description of 3D shapes. However, point-clouds are stored in irregular and unordered structures, which limits the direct use of segmentation algorithms such as Convolutional Neural Networks. The objective of our work is twofold: First, we aim to provide a full analysis of the PointNet architecture to illustrate which features are being extracted from the point-clouds. Second, to propose a new network architecture called IPC-Net to improve the state-of-the-art point cloud architectures. We show that IPC-Net extracts a larger set of unique features allowing the model to produce more accurate segmentations compared to the PointNet architecture. In general, our approach outperforms PointNet on every family of 3D geometries on which the models were tested. A high generalisation improvement was observed on every 3D shape, especially on the rockets dataset. Our experiments demonstrate that our main contribution, inter-point activation on the network's layers, is essential to accurately segment 3D point-clouds.

==> abstract.tex <==
\begin{abstract}

Over the last decade, the demand for better segmentation and classification algorithms in 3D spaces has significantly grown due to the popularity of new 3D sensor technologies and advancements in the field of robotics. Point-clouds are one of the most popular representations to store a digital description of 3D shapes. However,  point-clouds are stored in irregular and unordered structures, which limits the direct use of segmentation algorithms such as Convolutional Neural Networks.  The objective of our work is twofold: First, we aim to provide a full analysis of the PointNet architecture to illustrate which features are being extracted from the point-clouds. Second, to propose a new network architecture called IPC-Net to improve the state-of-the-art point cloud architectures. We show that IPC-Net extracts a larger set of unique features allowing the model to produce more accurate segmentations compared to the PointNet architecture. In general, our approach outperforms PointNet on every family of 3D geometries on which the models were tested. A high generalisation improvement was observed on every 3D shape, especially on the rockets dataset. Our experiments demonstrate that our main contribution, inter-point activation on the network's layers, is essential to accurately segment 3D point-clouds.
  %PointNet is one of the first Neural Networks architectures that addressed the problem of direct learning of 3D point-clouds. This architecture approximates symmetric functions to introduce order invariance in the point cloud and exploits spatial information between dimensions of the input space to extract global and local characteristic of each point in the cloud. However, PointNet ignores the inter spatial features that exists between neighbouring points within one segmentation. 
%  We conclude by stating that inter-point activation on the layers of the networks is essential to accurately segment 3D point-clouds. 
%    to compare our models with the PointNet architecture with different  3D geometry families of the shape database.  Our approach outperforms PointNet on  every  dataset  both the training and testing set of the PointNet model in 4 dataset of the ShapeNet database.  
% We solve the ..  in 3D D address the 
% The introduction of new technologies such as 3D printing, Virtual Reality
% (VR) and 3D sensor technologies has increased the demand for more geometric
% ?
%  Supported by organisation Doctiris-Innoviris-Brussels.
% 2
%  F. Gomez et al.
% manipulation methods. 3D Segmentation plays a big role in the field of geometry
% 
% The abstract should briefly summarize the contents of the paper in
% 15--250 words.

\begin{IEEEkeywords}
  Convolutional Neural Networks, Irregular Domains, Segmentations, Kernel visualisation
\end{IEEEkeywords}


% \keywords{Deep Learning \and \and Shape Analysis \and Computer vision \and Point cloud \and Segmentation \and Conditional Random Fields}
\end{abstract}


==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In pointNet++ the also arrived to the same conclusion  that the vanilla PoinNet does not considers inter-local point information.  They been exploiting the features at the dimension space however they do not exploit the characteristics that exist within neighbouring points.


==> results.tex <==
\section{Results}
